Contextual Data Augmentation for Task-Oriented Dialog Systems

Collection of annotated dialogs for training task-oriented dialog systems have been one of the key bottlenecks in improving current models. While dialog response generation has been widely studied on the agent side, it is not evident if similar generative models can be used to generate a large variety of, and often unexpected, user inputs that real dialog systems encounter in practice. Existing data augmentation techniques such as paraphrase generation do not take the dialog context into consideration. In this paper, we develop a novel dialog augmentation model that generates a user turn, conditioning on full dialog context. Additionally, with a new prompt design for language model, and output re-ranking, the dialogs generated from our model can be directly used to train downstream dialog systems. On common benchmark datasets MultiWoZ and SGD, we show that our dialog augmentation model generates high quality dialogs and improves dialog success rate by as much as $8\%$ over baseline.

==> BART.tex <==





% \begin{table*}[t]
%     \centering
%     \small
%     \begin{tabular}{l | l l | l p{1.4cm} l l}
%     \toprule
%         \textbf{EXPNAME} & \textbf{Completion} & \textbf{Success} & \textbf{BLEU} & \textbf{BERTScore} & \textbf{BLEURT} & \textbf{Perplexity} \\ 
%         \midrule
%         Baseline & 0.873 & 0.733 & ~ & ~ & ~ & ~ \\ \hline
%         Baseline with Aug. & 0.930 & 0.794 & 0.104 & 0.890 & -0.547 & 38.362 \\ \hline
%         Filter & \textbf{0.936} & 0.751 & 0.104 & 0.890 & -0.547 & 38.362 \\ \hline
%         Sys/Usr (colon) & 0.910 & 0.772 & 0.109 & 0.890 & -0.518 & 40.296 \\ \hline
%         Filter, Sys/Usr (colon) & 0.928 & \textbf{0.816} & 0.162 & 0.908 & -0.092 & 374.542 \\ \hline
%         Sys/Usr ("says") & 0.899 & 0.745 & 0.105 & 0.893 & -0.512 & 275.688 \\ \hline
%         Sys/Usr ("says"), SLOTS & 0.927 & 0.734 & 0.120 & 0.894 & -0.402 & 187.290 \\ \hline
%         Filter, Sys/Usr ("says"), Slots & 0.911 & 0.720 & 0.180 & 0.911 & -0.021 & 32.091 \\ \hline
%         Filter, Sys/Usr (colon), Slots & 0.928 & 0.732 & 0.177 & 0.909 & -0.054 & 32.394 \\
%         \bottomrule
%     \end{tabular}
%     \caption{\label{tab:BART-ablation}Results of the our BART dialog augmentation model and its ablations. First two columns show extrinsic evaluation metrics, while the remaining columns present intrinsic evaluation metrics.}
% \end{table*}

==> T5.tex <==
\section{Parameters}
\label{app:parameters}

In this section we discuss the parameters for our experiment in more details. Our models were implemented in PyTorch. We fine tune both BART (base) and T5 (base) models for 3 and 2 epochs respectively on the dialog augmentation task. We use batch size in $\{8, 16\}$, learning rate in $2 \times \{10^{-5}, 10^{-4}\}.$ For BART, we freeze the encoder and embeddings during training. During inference, for both models we use $4$ eval beams. For extrinsic evaluation, we train the Soloist \cite{SOLOIST:PengLLSLG21} model using default hyper-parameters using the original code\footnote{https://github.com/pengbaolin/soloist}. We train the model until the validation loss has decreased for $5$ consecutive evaluations (conducted every $2000$ steps). We train all models using a machine with single V100 GPU.

\midrule
        with Base T5 Augmentation & 0.927 & 0.742
 & 0.282 & 0.912 & -0.334 & 109.259 \\ \hline
        + $\langle user \rangle$/ $\langle system \rangle$ & 0.926 & 0.734 & 0.228 & 0.880 & -0.700 & 131.971 \\ \hline
        + "user:"/"system:" &  0.917 & 0.749 &  0.292 & 0.915 & -0.260 & 105.984 \\ \hline
        + "user/system says" &  &  &  0.290 & 0.914 & -0.277 & 112.066 \\ \hline
        + BS slots & & & 0.337 & 0.924 & -0.112 & 112.312 \\ \hline
        + filter &  &  &  0.360 & 0.925 & -0.0256 & 99.860 \\ \hline
        + filter + "user:"/"system:" &  &  &  0.366 & 0.926 & 0.017 & 98.744 \\ \hline
        + "user/system says" + BS Slots &  &  &  0.341 & 0.924 & -0.099 & 114.148  \\ \hline
        + filter + "user:"/"system:" + BS slots &  &  &  \textbf{0.427} & \textbf{0.936} & \textbf{0.165} & 110.206  \\ \hline
        
        
        
    \midrule
        w/ Base T5 Augmentation & 0.369 & 0.926 & -0.049 & 141.41 \\ \hline
        + "user:/ system:" & 0.369 & 0.926 & -0.045 & 133.41 \\ \hline
        + filter + "user:/ system:" & 0.491 & 0.942 & 0.268 & 122.12 \\ \hline
        + BS slots & 0.416 & 0.934 & 0.077 & 182.21 \\ \hline
        + "user:/ system:" + BS Slots & 0.370 & 0.925 & -0.127 & 203.25 \\ \hline
        \bottomrule
        
        
        
%% Soloist \cite{SOLOIST:PengLLSLG21} (upper bound)  & 0.714 & 0.505 & 0.845 & 0.692 \\

==> limitations.tex <==
\section{Limitations}

In this paper, we develop a new data augmentation model for task-oriented dialogs system. Despite its effectiveness, adding new augmented data to the training set increases the model training time. It is also not straightforward to determine the amount of dialogs to be augmented. Augmenting too few dialogs may be ineffective, while too many may slow down training and even be harmful performance wise by introducing too much noise and altering the original data distribution. Finally, there are some cases where the current turn has information that is not included in the other turns and the model does not capture it in the generation. Some portions of our approach mitigate this issue but it is still a partially solved problem that warrants more work.

==> related.tex <==
\section{Related Work} \label{app:related}

% General task-oriented dialog papers and neural network models
Task-oriented dialog models have been widely studied in the last two decades due to its commercial success in driving various voice assistants and chatbots. Traditionally, these models are divided into sub-components to accomplish individual tasks e.g. language understanding \cite{Hakkani-TurTCCG16,LiuL16,goo2018slot}, dialog state tracking \cite{MrksicSWTY17,ChenLWZT020}, dialog policy learning \cite{WenMBY17,GaoWPLL18}, and dialog response generation \cite{WenGMSVY15,ShenSLLNZAL17,ZhangSGCBGGLD20}. Recently, more end-to-end approaches have been developed which can jointly accomplish all sub-tasks \cite{HamLJK:20,SimpleTOD:Hosseini-AslMWY20,SOLOIST:PengLLSLG21,UBAR:YangLQ21}.    

% paraphrase generation with and with-out context
Lack of sufficient annotated training data still remains a fundamental challenge in developing spoken language understanding (SLU) and dialog models. Many data augmentation approaches have been explored to improve performance of SLU \cite{HouLCL:18,YooSL:19,ZhaoZY19,LinXZZZ21} and dialog models \cite{SongZH21}. However, these methods do not take into account any past or future dialog history.

Several approaches have also tried to incorporate dialog context in augmentation using various techniques e.g., paraphrase generation \cite{GaoZOY20}, data-balancing \cite{ZhangOY20}, reinforcement-learning \cite{YinSJCL20}, and graph based approach \cite{GrittaLI21}. 

% dialog response generation
Large-scale pre-trained language models have demonstrated superior performance for a wide range of NLP tasks including NLG \cite{GPT2:radford2019language,GPT3:BrownMRSKDNSSAA20,BART:LewisLGGMLSZ20,T5:RaffelSRLNMZLL20}. These models have also been successfully used to generate meaningful, and natural agent responses in task-oriented dialog systems, both with \cite{GuWWSY20,ZhangSGCBGGLD20,KaleR20} or without any dialog context \cite{PengZLLLZG20,KaleR20a,XuWKL20}. However, it is still largely unexplored if such pre-trained models can be used for effective augmentation of user utterances in a dialog to help improve end-to-end TOD model performance. In this paper, we attempt to throw some light on this question.  

% TODO review section added here by dax
%\todo{review section added here by dax}
%\dax{Additionally, response generation is typically a much more constrained problem due to its usage primarily being generation of System responses in an online context.  This means that response generation is rarely used for generating User utterances and mainly relies only on past information, since a response generation that requires future turns as input has few uses. Our system is intended for use in augmentation generation on both System and User turns. Also, we are able to leverage turns that appear after the current turn being augmented because when we are augmenting a dialog we typically have access to the entire dialog and are not augmenting online mid-dialog.}


% simulation based dialog generation


